Bug or Not? Bug Report Classification Using N-Gram IDF

Previous studies have found that a significant number of bug reports are misclassified between bugs and non-bugs, and that manually classifying bug reports is a time-consuming task. To address this problem, we propose a bug reports classification model with N-gram IDF, a theoretical extension of Inverse Document Frequency (IDF) for handling words and phrases of any length. N-gram IDF enables us to extract key terms of any length from texts, these key terms can be used as the features to classify bug reports. We build classification models with logistic regression and random forest using features from N-gram IDF and topic modeling, which is widely used in various software engineering tasks. With a publicly available dataset, our results show that our N-gram IDF-based models have a superior performance than the topic-based models on all of the evaluated cases. Our models show promising results and have a potential to be extended to other software engineering tasks.

==> sections/result_old.tex <==
N-gram IDF \cite{shirakawa2015n} is a theoretical extension of IDF for handling word and phrases of any length by comparing weights among N-grams of any length of N.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Result}\label{sec:result}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{N-gram IDF-based model performance}
Table \ref{table:fold_result} and Table \ref{table:train_result} show the evaluation result by 10-fold cross-validation setup and training - testing setup respectively. The first column indicates the text processing technique that was used to train the model. For the other columns, four consecutive columns are grouped into a set of study projects. Each set reports the performance of a classification model that employed one of the two classifier algorithms. As we see in Table \ref{table:fold_result}, logistic regression and random forest models yield a similar classifying performance range for each study project. The F-measure score varies between  0.80 - 0.81, 0.77 - 0.80, 0.82 - 0.88, and 0.79 - 0.81 for HTTPClient, Jackrabbit, Lucene, and Cross Project respectively for the 10-fold cross-validation testing method. For the another testing method, as we see in Table \ref{table:train_result}, the F-measure score varies between 0.68 - 0.69, 0.62 - 0.64, 0.68 - 0.73, and 0.65 - 0.67 for HTTPClient, Jackrabbit, Lucene, and Cross Project respectively.
	\par According to the numerical result, we conclude that N-gram IDF-based classification models are able to classify types of bug reports with significant performance and when considering the classification techniques, both logistic regression and random forest models seem to have an opportunity to be further developed to achieve higher classification performance.


\subsection{N-gram IDF based vs Topic-based Model}
In this subsection, we compare the classifying performance between N-gram IDF-based and topic-based model. To build a topic-based classification model, we follow the methodology conducted on the previous study \cite{pingclasai2013classifying}. To construct a model, we build a collection of topic membership vectors with 50 as a number of topics. Finally, we train the classification models with two classifier algorithms; logistic regression and random forest tree before evaluating the performance of each model.
	\par Table \ref{table:fold_result} and Table \ref{table:train_result} also show the performance comparison between topic-based and N-gram IDF-based classification models based. We see that N-gram IDF-based model slightly outperforms topic-based model in all of cases.
    
\subsection{N-gram IDF-based technique}
\input{table/n_gram_words.tex}

	Table \ref{table:n_gram_words} shows the example of N-gram words that were used as features for classification process. Since N-gram IDF can extract all of valid N-gram words of any length, N-gram IDF is capable of capturing the text structure in a sequential order. As we see in Table \ref{table:n_gram_words}, the N-gram words that were selected as features for mining process vary in both contexts and length of words, such as, \textit{how to reproduce} and \textit{demonstrate the problem} which are contexts in natural language, \textit{concurrentmodificationexception} and \textit{stringindexoutofboundsexception} which are contexts in programming syntax. Therefore, N-gram IDF can capture the word structure in both natural language context and programming syntax context with any length of the word.  With the strong point of N-gram IDF, our proposed N-gram IDF classification technique can be further developed not only to be used on the bug report classification task, but also on the other software engineering tasks.
	\par Technically, a time that our technique take to create and train a classification model depends on the size of document corpus. However, in a case of all required tools and dataset are provided with all of the necessary variables, we can complete the whole process starting from the scratch within a few hours. Therefore, our technique can help developers to accelerate their development process by reducing their in bug reports inspection process as they do not need to waste much effort and time on the manual bug report classification process. 

==> table/comparision_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{weighted F-measure value comparision table between topic-based and n-gram idf based classification models}
\label{table:performance_comparision}
\begin{tabular}{|l|l|c|c|c|c|c|c|}
\hline
 & \textbf{} & \multicolumn{3}{c|}{\textbf{10-fold cross validation}} & \multicolumn{3}{c|}{\textbf{Training set \& Testing set (top 1\% feature)}} \\ \cline{3-8} 
 & \textbf{} & \multicolumn{1}{l|}{\textbf{Naive Bayes}} & \multicolumn{1}{l|}{\textbf{Logistic Regression}} & \multicolumn{1}{l|}{\textbf{Random Forest}} & \multicolumn{1}{l|}{\textbf{Naive Bayes}} & \multicolumn{1}{l|}{\textbf{Logistic Regression}} & \multicolumn{1}{l|}{\textbf{Random Forest}} \\ \hline
 & \textbf{Topic-based} & 0.724 & 0.739 & 0.721 & 0.504 & 0.516 & 0.493 \\
\multirow{-2}{*}{\textbf{HTTPClient}} & \cellcolor[HTML]{C0C0C0}\textbf{N-gram IDF Based} & \cellcolor[HTML]{C0C0C0}0.715 & \cellcolor[HTML]{C0C0C0}0.805 & \cellcolor[HTML]{C0C0C0}0.814 & \cellcolor[HTML]{C0C0C0}0.589 & \cellcolor[HTML]{C0C0C0}0.687 & \cellcolor[HTML]{C0C0C0}0.698 \\ \hline
 & \textbf{Topic-based} & 0.742 & 0.744 & 0.717 & 0.453 & 0.511 & 0.520 \\
\multirow{-2}{*}{\textbf{Jackrabbit}} & \cellcolor[HTML]{C0C0C0}\textbf{N-gram IDF Based} & \cellcolor[HTML]{C0C0C0}0.662 & \cellcolor[HTML]{C0C0C0}0.805 & \cellcolor[HTML]{C0C0C0}0.771 & \cellcolor[HTML]{C0C0C0}0.534 & \cellcolor[HTML]{C0C0C0}0.646 & \cellcolor[HTML]{C0C0C0}0.625 \\ \hline
 & \textbf{Topic-based} & 0.757 & 0.766 & 0.756 & 0.474 & 0.562 & 0.566 \\
\multirow{-2}{*}{\textbf{Lucene}} & \cellcolor[HTML]{C0C0C0}\textbf{N-gram IDF based} & \cellcolor[HTML]{C0C0C0}0.515 & \cellcolor[HTML]{C0C0C0}0.884 & \cellcolor[HTML]{C0C0C0}0.823 & \cellcolor[HTML]{C0C0C0}0.307 & \cellcolor[HTML]{C0C0C0}0.731 & \cellcolor[HTML]{C0C0C0}0.680 \\ \hline
 & \textbf{Topic-based} & 0.709 & 0.724 & 0.712 & 0.456 & 0.592 & 0.538 \\
\multirow{-2}{*}{\textbf{Cross Project}} & \cellcolor[HTML]{C0C0C0}\textbf{N-gram IDF based} & \cellcolor[HTML]{C0C0C0}0.674 & \cellcolor[HTML]{C0C0C0}0.814 & \cellcolor[HTML]{C0C0C0}0.792 & \cellcolor[HTML]{C0C0C0}0.358 & \cellcolor[HTML]{C0C0C0}0.658 & \cellcolor[HTML]{C0C0C0}0.670 \\ \hline
\end{tabular}
\end{table*}

==> table/n_gram_table.tex <==
\begin{table*}[]
\centering
\caption{Weighted F-measure of the N-gram IDF based classification models separated by classifier algorithm and testing method}
\label{table:n-gram_result}
\begin{tabular}{|l|c|c|c|c|c|c|}
\hline & \multicolumn{3}{c|}{\textbf{10-fold cross validation}} & \multicolumn{3}{c|}{\textbf{Training set \& Testing set (top 1\% feature)}} \\ 
\cline{2-7}  & \multicolumn{1}{l|}{\textbf{Naive Bayes}} & \multicolumn{1}{l|}{\textbf{Logistic Regression}} & \multicolumn{1}{l|}{\textbf{Random Forest}} & \multicolumn{1}{l|}{\textbf{Naive Bayes}} & \multicolumn{1}{l|}{\textbf{Logistic Regression}} & \multicolumn{1}{l|}{\textbf{Random Forest}} \\ 
\hline
\textbf{HTTPClient} & 0.715 & 0.805 & 0.814 & 0.589 & 0.687 & 0.698 \\
\textbf{Jackrabbit} & 0.662 & 0.805 & 0.771 & 0.534 & 0.646 & 0.625 \\
\textbf{Lucene} & 0.515 & 0.884 & 0.823 & 0.307 & 0.731 & 0.680 \\
\textbf{Cross Project} & 0.674 & 0.814 & 0.792 & 0.358 & 0.658 & 0.670 \\ 
\hline
\end{tabular}
\end{table*}

==> table/n_gram_words2.tex <==
\begin{table}[]
\centering
\caption{Example of N-gram words that were utilized as features}
\label{table:n_gram_words}
\begin{tabular}{|l|l|}
\hline
concurrentmodificationexception & how to reproduce \\ \hline
stringindexoutofboundsexception & is this bug      \\ \hline
nullpointerexception            & deadlock in      \\ \hline
demonstrate the problem         & test showing the \\ \hline
\end{tabular}
\end{table}
